High-Quality Hypergraph Partitioning

This paper considers the balanced hypergraph partitioning problem, which asks for partitioning the vertices into $k$ disjoint blocks of bounded size while minimizing an objective function over the hyperedges. Here, we consider the most commonly used connectivity metric. We describe our open source hypergraph partitioner KaHyPar which is based on the successful multi-level approach -- driving it to the extreme of one level for (almost) every vertex. Using carefully designed data structures and dynamic update techniques, this approach offers a very good time-quality tradeoff. We present two preprocessing techniques -- pin sparsification using locality sensitive hashing and community detection based on the Louvain algorithm. The community structure is used to guide the coarsening process that incrementally contracts vertices. Portfolio-based partitioning of the contracted hypergraph already achieves good initial solutions. While reversing the contractions, a combination of highly-localized direct $k$-way local search and flow-based techniques that take a more global view, refine the partition to achieve high quality. Optionally, a memetic algorithm evolves a pool of solution candidates to obtain even higher quality. We evaluate KaHyPar on a large set of instances from a wide range of application domains. With respect to quality, KaHyPar outperforms all previously considered systems that can handle large hypergraphs such as hMETIS, PaToH, Mondriaan, or Zoltan. KaHyPar is also faster than most of these systems except for PaToH which represents a different speed-quality tradeoff. The results even extend to the special case of graph partitioning, where specialized systems such as KaHIP should have an advantage.

==> img/jea_19/preamble-ipe.tex <==
% ---[ Finalizing ]-------------------------------------------------------------

% final book print
\newif\ifFinalPrint

% ------------------------------------------------------------------------------

% this enables big black bars on overlong lines.
\setlength\overfullrule{14pt}

% always enable synctex
\synctex=1

% font encoding: 8bit encoding
\usepackage[T1]{fontenc}
% input encoding: utf8 support
\usepackage[utf8]{inputenc}
% language settings: British English, New German
\usepackage{babel}

%\usepackage{csquotes}

% Latin Modern font
\usepackage{lmodern}
% palatino "sans-"serif font
\renewcommand{\sfdefault}{ppl}
% extra math font
\usepackage{dsfont}
% another teletype font
\usepackage[nott]{inconsolata}
\def\consolata#1{\begingroup\fontfamily{zi4}\selectfont{#1}\endgroup}

% dagger symbols
\usepackage{textcomp}

% math symbols
\usepackage{amsmath,amsfonts,amssymb}
% small fractions in running text
\usepackage{nicefrac}
% text symbols
\usepackage{textcomp}
% extra math tools
\usepackage{mathtools}
% better arrays
\usepackage{array}
% better tabulars
\usepackage{tabularx,longtable}
% for tabulars with footnotes
\usepackage[flushleft]{threeparttable}
% for rotate tables
\usepackage{rotating}
% \begin{commment}
\usepackage{verbatim}
% latex hacks, e.g. robustify
\usepackage{etoolbox}
% arithmetic
\usepackage{calc}
% \hdashline
\usepackage{arydshln}
% varwidth paragraphs
\usepackage{varwidth}
% after page
\usepackage{afterpage}

% nicer text layout
\usepackage{microtype}

% allow graphics
\usepackage{graphicx}

% allow colors
\usepackage{xcolor}

\usepackage{tabstackengine}

% adaptive whitespace
\usepackage{xspace}

% chapter headers
\usepackage[explicit]{titlesec}

% allow hyperlinks
\usepackage{hyperref}
% setup hyperref
\hypersetup{
  pdftitle={High Quality Hypergraph Partitioning},
  pdfauthor={Sebastian Schlag},
  pdfsubject={hypergraphs, partitioning, dissertation},
  % hyperlinks in original color
  colorlinks=false,
  % hyperlinks without border
  pdfborder={0 0 0},
  % open all bookmark folders
  bookmarksopen=true,
  % enumerate bookmarks
  bookmarksnumbered=true,
  % allow links to line break
  breaklinks=true,
  unicode=true
}
\providecommand\phantomsection{} 

\makeatletter 
\newcommand{\textlabel}[2]{% 
  \protected@edef\@currentlabel{#1}% Set target label 
  \phantomsection% Correct hyper reference link 
  #1\label{#2}% Print and store label 
} 
\makeatother 

% change chapter counters to reset within each part
% \usepackage{chngcntr}
% \counterwithin{chapter}{part}

% page layout
\usepackage{scrpage2}
% better integration of hyperref, listings, float
\usepackage{scrhack}

% place floats exactly here [H]
\usepackage{float}
% fraction of page for top floats
\renewcommand{\topfraction}{0.8}
\renewcommand{\floatpagefraction}{0.8}

% caption for sub-elements
\usepackage[font=normalsize, labelformat=simple, list=true]{subcaption}
\renewcommand\thesubfigure{\,(\alph{subfigure})}

\usepackage{pdflscape}

% nicer tables
\usepackage{booktabs}
% table cells spanning rows
\usepackage{multirow}

% break long citations
\usepackage{breakcites}


% nice listings
% \usepackage[chapter]{algorithm}
% general settings for pseudo-code algorithms
% \usepackage{algpseudocode}

% fix for standalone drawing: add chapter counter
% \ifstandalone
%   \newcounter{chapter}
% \fi

% \ifstandalone\else

% algorithm formatting
% ours:
% \usepackage[
% % environment is algorithm2e instead of algorithms and \listofalgorithmes
% algo2e,
% % algo numbering within part, chapter or section
% algochapter,
% % layout of the algorithm
% ruled,vlined,
% % auto numbering of the algorithm's lines
% linesnumbered,
% % don't use relsize package (useful if it breaks the compatibily)
% norelsize]{algorithm2e}
% \DontPrintSemicolon
% \SetAlCapHSkip{0pt}
% \IncMargin{-\parindent}
% \SetProgSty{}
% \SetFuncSty{}
% \SetArgSty{}
% \def\listalgorithmcfname{List of Algorithms}
% \def\algorithmautorefname{Algorithm}

% % alias \tcp*{} to \Rem{} for pseudo-code comments, who knows what tcp* stands for?
% \newcommand{\Rem}[1]{\tcp*{#1}}
% % for pseudo-code comments inside () clauses, without line break
% \newcommand{\Remi}[1]{\tcp*[f]{#1}}
% % change C++ comments formatting
% \SetKwComment{tcp}{{\upshape{}/\!/}\,}{}%
% \SetCommentSty{textit}

% % Custom pseudo-code functions
% \SetKwProg{Function}{Function}{}{}
% \SetKwFunction{LCPCompare}{LCP-Compare}

% % C/C++ style increment and decrement (with nicer styling)
% \newcommand{\Inc}{{++}}
% \newcommand{\Dec}{{--}}

% \fi

% listings
\usepackage{listings}
\lstset{
  language=C++,
  columns=fullflexible,
  basicstyle={\ttfamily},
  keywordstyle={\bfseries\color{dblue}},
  emphstyle={\color{dred}},
  aboveskip=0pt,
  belowskip=0pt,
}

\AtBeginDocument{%
  \renewcommand{\thelstlisting}{\arabic{chapter}.\arabic{lstlisting}}%
}

% Timo's TODOs
\newcommand{\TODO}[1]{%
  %{\sffamily\textbf{TODO}}%
  {{\sffamily\textbf{TODO}}[\textcolor{red}{\textit{#1}}]}%
  \marginpar{%
    %\raggedright\footnotesize\itshape{#1}\par%
    \raggedright\sffamily\textcolor{red}{\textbf{TODO}}\par%
  }}

% % format colon nicely in math typeset
% \mathchardef\ordinarycolon\mathcode`\:
% \mathcode`\:=\string"8000
% \begingroup \catcode`\:=\active
% \gdef:{\mathrel{\mathop\ordinarycolon}}
% \endgroup

% change \footnote{} style to use symbols
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}

% a command to print the footnote symbols, no idea why this does not exist.
\makeatletter
\newcommand{\fnsym}[1]{%
  \@fnsymbol{#1}%
}
\makeatother

% \textvtt{abc} - variable-width teletype with nicer literal underscores
\begingroup
\catcode`_=\active
\gdef\ActivateUnderscore{%
  % magic to replace underscore with a macro
  \def_{\texttt{\textunderscore}}%
  \catcode`\_=\active
}
\endgroup
\gdef\textvtt#1{%
  \begingroup\text{%
    \ActivateUnderscore{%
      \fontfamily{lmvtt}\selectfont{%
        \scantokens{#1\endinput}}}}%
  \endgroup}

%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%    KIT Colors                                                                %

\definecolor{KITgreen}  {cmyk/RGB}{  1,0,.60,0 /   0,150,130} % 100% green
\definecolor{KITgreen70}{cmyk/RGB}{.70,0,.42,0 /  76,181,167} %  70% green
\definecolor{KITgreen50}{cmyk/RGB}{.50,0,.30,0 / 127,202,192} %  50% green
\definecolor{KITgreen30}{cmyk/RGB}{.30,0,.18,0 / 178,223,217} %  30% green
\definecolor{KITgreen15}{cmyk/RGB}{.15,0,.09,0 / 217,239,236} %  15% green

\definecolor{KITblue}  {cmyk/RGB}{.80,.500,0,0 /  70,100,170} % 100% blue
\definecolor{KITblue70}{cmyk/RGB}{.56,.350,0,0 / 125,146,195} %  70% blue
\definecolor{KITblue50}{cmyk/RGB}{.40,.250,0,0 / 162,177,212} %  50% blue
\definecolor{KITblue30}{cmyk/RGB}{.24,.150,0,0 / 199,208,229} %  30% blue
\definecolor{KITblue15}{cmyk/RGB}{.12,.075,0,0 / 227,232,242} %  15% blue

\definecolor{KITblack}  {cmyk/RGB}{0,0,0,  1 /   0,  0,  0} % 100% black
\definecolor{KITblack70}{cmyk/RGB}{0,0,0,.70 /  77, 77, 77} %  70% black
\definecolor{KITblack50}{cmyk/RGB}{0,0,0,.50 / 128,128,128} %  50% black
\definecolor{KITblack30}{cmyk/RGB}{0,0,0,.30 / 179,179,179} %  30% black
\definecolor{KITblack15}{cmyk/RGB}{0,0,0,.15 / 217,217,217} %  15% black

\definecolor{KITpalegreen}{cmyk/RGB}{.6,0,1,0 / 130,190,60}
\colorlet{KITpalegreen70}{KITpalegreen!70}
\colorlet{KITpalegreen50}{KITpalegreen!50}
\colorlet{KITpalegreen30}{KITpalegreen!30}
\colorlet{KITpalegreen15}{KITpalegreen!15}

\definecolor{KITyellow}{cmyk/RGB}{0,.05,1,0 /  250,230,20}
\colorlet{KITyellow70}{KITyellow!70}
\colorlet{KITyellow50}{KITyellow!50}
\colorlet{KITyellow30}{KITyellow!30}
\colorlet{KITyellow15}{KITyellow!15}

\definecolor{KITorange}{cmyk/RGB}{0,.45,1,0 / 220,160,30}
\colorlet{KITorange70}{KITorange!70}
\colorlet{KITorange50}{KITorange!50}
\colorlet{KITorange30}{KITorange!30}
\colorlet{KITorange15}{KITorange!15}

\definecolor{KITbrown}{cmyk/RGB}{.35,.5,1,0 / 160,130,50}
\colorlet{KITbrown70}{KITbrown!70}
\colorlet{KITbrown50}{KITbrown!50}
\colorlet{KITbrown30}{KITbrown!30}
\colorlet{KITbrown15}{KITbrown!15}

\definecolor{KITred}{cmyk/RGB}{.25,1,1,0 / 160,30,40}
\colorlet{KITred70}{KITred!70}
\colorlet{KITred50}{KITred!50}
\colorlet{KITred30}{KITred!30}
\colorlet{KITred15}{KITred!15}

\definecolor{KITlilac}{cmyk/RGB}{.25,1,0,0 / 160,0,120}
\colorlet{KITlilac70}{KITlilac!70}
\colorlet{KITlilac50}{KITlilac!50}
\colorlet{KITlilac30}{KITlilac!30}
\colorlet{KITlilac15}{KITlilac!15}

\definecolor{KITcyanblue}{cmyk/RGB}{.9,.05,0,0 / 80,170,230}
\colorlet{KITcyanblue70}{KITcyanblue!70}
\colorlet{KITcyanblue50}{KITcyanblue!50}
\colorlet{KITcyanblue30}{KITcyanblue!30}
\colorlet{KITcyanblue15}{KITcyanblue!15}

\definecolor{KITseablue}{cmyk/RGB}{.35294,.23529,0,.45097 / 50,80,140}
\definecolor{KITwhite}{cmyk/RGB}{0,0,0,0 / 255, 255, 255}
\definecolor{KITdarkblue}{cmyk/RGB}{1.0,1.0,0,0.6 / 0, 0, 102}

\colorlet{KITolive}{KITpalegreen}
\colorlet{KITmagenta}{KITlilac}
\colorlet{KITcyan}{KITcyanblue}

\colorlet{dpurple}{violet}
\colorlet{dgreen}{KITgreen}
\colorlet{dblue}{KITblue!60!blue}
\colorlet{dred}{KITred!60!red}

\def\balert#1{\textcolor{dblue}{#1}}
\def\galert#1{\textcolor{dgreen}{#1}}
\def\ralert#1{\textcolor{red}{#1}}

%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%    Custom Layout Settings                                                    %

% do not uppercase all \markleft{} and \markboth{} page titles
\def\MakeMarkcase#1{#1}

% ---[ Part ]-------------------------------------------------------------------

%\definecolor{chaptergrey}{rgb}{0.6,0,0}
\definecolor{chaptergrey}{rgb}{0,0,0}

\newenvironment{savequote}[1][10cm]{%
  \begin{lrbox}{\quotebox}
    \begin{minipage}[t]{#1}\footnotesize\itshape\ignorespaces}{%
      \unskip\end{minipage}\end{lrbox}
  \global\setbox\quotebox\copy\quotebox
  \ignorespacesafterend}
\newcommand{\qauthor}[1]{%
  \par\smallskip
  {\raggedleft\upshape #1\qquad\hbox{}\par}\bigskip}
\newcommand{\qsetcnfont}[1]{%
    \renewcommand*{\defaultcnfont}{#1}}
\newsavebox{\quotebox}

\newenvironment{partabstract}[1][0.9\textwidth]{%
  \begin{lrbox}{\partabstractbox}
    \begin{minipage}[t]{#1}\normalfont\itshape\ignorespaces}{%
      \unskip\end{minipage}\end{lrbox}
  \global\setbox\partabstractbox\copy\partabstractbox
  \ignorespacesafterend}
\newsavebox{\partabstractbox}

\titleformat{name=\part}[display]{%
  % format:
  \thispagestyle{empty}\enlargethispage{2cm}}{%
  % label:
  \vbox to 110pt{\copy\quotebox\vss}%
  \vbox{%
    \raggedleft
    \fontfamily{ppl}\fontsize{100}{100}\selectfont
    \hfill\textcolor{chaptergrey}{\thepart}\newline
    \hfill\bfseries\fontfamily{ppl}\fontsize{20}{26}\selectfont#1%
  }
  \vspace{3em}
  \vbox{\centerline{\copy\partabstractbox}}%
}{%
  % sep:
  0pt}{%
  % before-body-code:
  \vspace{1pc}%
}
\titlespacing*{\part}{0pt}{0pt}{0pt}

% ---[ Chapter ]----------------------------------------------------------------

\titleformat{name=\chapter}[display]{
  % format/label/sep:
  \sffamily\bfseries\fontsize{20}{22}\selectfont}{}{0pt}{
  % before-body-code:
  \begingroup
  \setlength{\unitlength}{1mm}
  \renewcommand{\gobble}[1]{}
  \begin{picture}(25,0)(0,5)
    \ifnumless{\thechapter}{10}{%
      \put(0,15){\line(1,0){\dimexpr\textwidth-15\unitlength\relax\gobble}}%
    }{%
      \put(0,15){\line(1,0){\dimexpr\textwidth-30\unitlength\relax\gobble}}
    }
    \put(100,1){\makebox(30,20)[r]{%
        \fontsize{72}{72}\selectfont\thechapter}}
    \put(0,15){%
      \makebox(\dimexpr\textwidth-20\unitlength\relax\gobble,\ht\strutbox\gobble)[l]{%
        \normalsize\chapapp~\thechapter}}
    \ifnumless{\thechapter}{10}{%
      \put(3,10){\parbox[t]{%
          \dimexpr\textwidth-19\unitlength\relax}{\raggedright\color{black} #1}}
    }{
      \put(3,10){\parbox[t]{%
          \dimexpr\textwidth-34\unitlength\relax}{\raggedright\color{black} #1}}
    }
  \end{picture}
  \endgroup
}
\titleformat{name=\chapter,numberless}[display]{
  % format/label/sep:
  \sffamily\bfseries\fontsize{20}{22}\selectfont}{}{0pt}{
  % before-body-code:
  \begingroup
  \vbox{%
    \raggedleft #1%
  }
  \endgroup
}

\titlespacing{name=\chapter}{0pt}{0pt}{50pt}
\titlespacing{name=\chapter,numberless}{0pt}{0pt}{20pt}

\makeatletter
% environment for chapter abstracts
\newenvironment{chapterabstract}{
  \bgroup
  \itshape
  \list{}{\leftmargin0.75cm\rightmargin\leftmargin}
\item\relax
}{
  \endlist
  \@afterindentfalse
  \@afterheading
  \egroup
}
\makeatother

% ---[ Paragraph ]--------------------------------------------------------------

\titleformat{\paragraph}[runin]{%
  \normalfont\normalsize\bfseries}{\theparagraph}{0em}{#1.}{}
\titlespacing*{\paragraph}{0pt}{\medskipamount}{1em}

% header / footer style
% \ifstandalone\else
%   \pagestyle{scrheadings}
%   \setkomafont{pageheadfoot}{\normalfont\rmfamily}
%   \setkomafont{pagenumber}{\normalfont\rmfamily}
%   \setheadsepline{.4pt}
%   \automark[section]{chapter}
% \fi

% nicer captions
\usepackage{caption}

% caption style (general)
\captionsetup*{
  format=plain,
  labelfont={bf,up},
  margin=10pt,
}

% caption style (sub-elements)
\captionsetup*[sub]{
  format=plain,
  labelfont={bf,up},
  margin=10pt,
  skip=2pt
}

\usepackage{mdframed}
\definecolor{grisframe}{gray}{0.95}
\newmdenv[
  topline=false,
  bottomline=false,
  rightline=false,
  linewidth=3pt,
  linecolor=gray,
  innertopmargin=0pt,
  innerbottommargin=0pt,
  splitbottomskip=0pt,
  skipabove=.5\baselineskip,
  skipbelow=.5\baselineskip
]{siderules}

% ---[ better array column types ]----------------------------------------------

\newcolumntype{L}[1]{>{%
    \raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{%
    \centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{%
    \raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcolumntype{Y}{>{%
    \raggedleft\arraybackslash}X}

\newcolumntype{H}{@{}>{\iffalse}l<{\fi}}

% ---[ better enumerations ]----------------------------------------------------

\usepackage{enumitem}

% smaller margin for list environments
\setlist[itemize]{leftmargin=1.5em}
\setlist[enumerate]{leftmargin=1.5em}
\setlist[description]{leftmargin=1.5em}

\setlist[itemize]{topsep=0pt, labelsep=1ex}
\setlist[enumerate]{topsep=0pt, labelsep=1ex}
\setlist[description]{font=\normalfont,topsep=0pt}

\setlist[enumerate,1]{label=(\roman*), ref={\thetheorem\,(\roman*)}}
\setlist[enumerate,2]{label=(\alph*), ref={\thetheorem\,(\alph*)}}

% % also break URLs at any letter and number
% \expandafter\def\expandafter\UrlBreaks\expandafter{%
%   % normally = \do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]\do\)\do\,\do\?\do\'\do\+\do\=\do\#
%   \UrlBreaks%
%   \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
%   \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
%   \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
%   \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
%   \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
%   \do\Y\do\Z\do\0\do\1\do\2\do\3\do\4\do\5\do\6\do\7%
%   \do\8\do\9%
% }


% ---[ flow symbols ]----------------------------------------------------
\usepackage{stmaryrd}



%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%                                                                              %

% ---[ Macros ]-----------------------------------------------------------------

% round up
\newcommand{\ceil}[1]{\ensuremath{\lceil #1 \rceil}}
% roundd down
\newcommand{\floor}[1]{\ensuremath{\lfloor #1 \rfloor}}

% \arr{...} denotes an (ordered) array
\newcommand{\arr}[1]{[\, #1 \,]}
% \arrc{...} denotes an (ordered) array with less space
\newcommand{\arrc}[1]{[#1]}
% \arro{...} denotes an (ordered) right-open array
\newcommand{\arro}[1]{[\, #1 \kern.1em )}
% \set{...} denotes an (unordered) set
\newcommand{\set}[1]{\left\{ #1\right\}}
% \seq{...} sequence <...>
\newcommand{\seq}[1]{\left\langle #1\right\rangle}

% Landau Big-O
\newcommand{\Oh}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\oh}[1]{\ensuremath{\mathrm{o}(#1)}\xspace}
\newcommand{\Om}[1]{\ensuremath{\Omega(#1)}\xspace}
\newcommand{\om}[1]{\ensuremath{\omega(#1)}\xspace}
\newcommand{\Th}[1]{\ensuremath{\Theta(#1)}\xspace}

% Landau Big-O vertically expanding
\newcommand{\vOh}[1]{\ensuremath{\mathcal{O}\left(#1\right)}\xspace}
\newcommand{\voh}[1]{\ensuremath{\mathrm{o}\left(#1\right)}\xspace}
\newcommand{\vOm}[1]{\ensuremath{\Omega\left(#1\right)}\xspace}
\newcommand{\vom}[1]{\ensuremath{\omega\left(#1\right)}\xspace}
\newcommand{\vTh}[1]{\ensuremath{\Theta\left(#1\right)}\xspace}

% mathmatical operators
\newcommand{\xor}{\mathbin{\oplus}}

\def\mathsc#1{\ensuremath{\text{\textsc{#1}}}}


%\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{wasysym}
\newcommand{\no}{$\Circle$}%
\newcommand{\yes}{$\CIRCLE$}%
\newcommand{\yesno}{$\LEFTcircle$}
\newcommand{\ymark}{\ding{51}}%


\newcommand{\Partition}{\ensuremath{\mathrm{\Pi}}}%
\newcommand{\neighbors}{\ensuremath{\mathrm{\Gamma}}}%
\newcommand{\incnets}{\ensuremath{\mathrm{I}}}%
\newcommand{\pinsinpart}{\ensuremath{\mathrm{\Phi}}}
\newcommand{\adjblocks}{\ensuremath{\mathrm{B}}}
\newcommand{\con}{\ensuremath{\lambda}}
\newcommand{\conset}{\ensuremath{\Lambda}}
\newcommand{\frompart}{\ensuremath{V_{\text{\upshape from}}}}
\newcommand{\topart}{\ensuremath{V_{\text{\upshape to}}}}
\newcommand{\frompq}{\ensuremath{P_{\text{\upshape from}}}}
\newcommand{\topq}{\ensuremath{P_{\text{\upshape to}}}}
\newcommand{\fromgain}{\ensuremath{g_{\text{\upshape from}}}}
\newcommand{\togain}{\ensuremath{g_{\text{\upshape to}}}}

\newcommand{\ocut}{\ensuremath{\mathfrak{f}_c(\Partition)}}%
\newcommand{\ocon}{\ensuremath{\mathfrak{f}_\lambda(\Partition)}}%
\newcommand{\osoed}{\ensuremath{\mathfrak{f}_s(\Partition)}}%
\newcommand{\orc}{\ensuremath{\mathfrak{f}_{rc}(\Partition)}}%
\newcommand{\osc}{\ensuremath{\mathfrak{f}_{sc}(\Partition)}}%


% \SetKw{Continue}{continue}
% \SetKwFunction{Activate}{Activate}
% \SetKwFunction{rate}{rate}
% \SetKwFunction{coarsen}{coarsen}
% \SetKwFunction{DeltaGainUpdate}{DeltaGainUpdate}
% \SetKwFunction{UpdateGainCache}{UpdateGainCache}

\usepackage{etoolbox,siunitx}
\sisetup{detect-weight=true,detect-inline-weight=math}
\robustify\bfseries

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\ALL}{All}
\newcommand{\Dual}{Dual}
\newcommand{\Primal}{Primal}
\newcommand{\ISPD}{ISPD98}
\newcommand{\Literal}{Literal}
\newcommand{\SPM}{SPM}
\newcommand{\DAC}{DAC2012}

\newcommand{\KaHyPar}[1]{KaHyPar-#1}
\newcommand{\KaHyParConfig}[2]{KaHyPar-#1$_\text{(#2)}$}
\newcommand{\hMetis}[1]{hMetis-#1}
\newcommand{\PaToH}[1]{PaToH-#1}

\newcommand{\FlowVariant}[3]{(#1\text{F},#2\text{M},#3\text{LS})}
\newcommand{\Constant}[1]{\textsc{Constant#1}}


\DeclareMathOperator*{\argmax}{arg\,max}%

\newcommand*\rot{\rotatebox{90}}
%\newcommand*\OK{\ding{51}}
\newcommand*\OK{\yes}
% \newcommand{\NOK}{\ding{55}}%
\newcommand{\NOK}{\no}%

% \usepackage{relsize}
% https://tex.stackexchange.com/questions/4302/prettiest-way-to-typeset-c-cplusplus
% \newcommand\CC{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}}
\newcommand\CC{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}}


% ---[ Theorem Environments ]---------------------------------------------------

\usepackage[amsmath,thmmarks,hyperref]{ntheorem}

% \renewtheoremstyle{break}%
%   {\labelsep=0pt\item[\rlap{\vbox{\hbox to \textwidth{\upshape\bfseries ##1\ ##2\hskip 0pt plus 1fil}\hbox{\strut}}}]}%
%   {\labelsep=0pt\item[\rlap{\vbox{\hbox to \textwidth{\upshape\bfseries ##1\ ##2\ (##3\unskip)\hskip 0pt plus 1fil}\hbox{\strut}}}]}

\renewtheoremstyle{nonumberplain}%
  {\labelsep=0pt\item[\itshape ##1.\quad]}%
  {\labelsep=0pt\item[\itshape ##1.\ (##3)\quad]}

\theoremstyle{break}
\theorembodyfont{\itshape}
\theoremseparator{\smallskip}
\theorempreskip{\bigskipamount}
\theorempostskip{\medskipamount}

% \newtheorem{theorem}{Theorem}[chapter]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{observation}[theorem]{Observation}

% proof environment
\theoremstyle{nonumberplain}
\theoremheaderfont{\itshape}
\theoremsymbol{\ensuremath{\;\square}}
\theorempreskip{}
\theorempostskip{}
\theorembodyfont{\normalfont}
\newtheorem{proof}{Proof}

% make text in \textbf{} also bold in math mode
\makeatletter
\DeclareRobustCommand*{\bfseries}{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont
  \boldmath\let\mathbbnormal=\mathbb\let\mathbb=\mathbbm
}
\makeatother

\newcommand*{\skippingparagraph}{\par\vspace{.5\baselineskip}\noindent}


==> img/jea_19/preamble.tex <==
% ---[ TikZ externalize ]-------------------------------------------------------

\usepackage{tikz}
\usetikzlibrary{external}

\tikzset{
  external/optimize=true,
  % external/mode=list and make,
  % external/prefix={figures/},
  external/figure name=figure_\thechapter_,
}
\tikzexternalize

% ---[ Finalizing ]-------------------------------------------------------------

% final book print
\newif\ifFinalPrint

% ------------------------------------------------------------------------------

% this enables big black bars on overlong lines.
\setlength\overfullrule{14pt}

% always enable synctex
\synctex=1

% font encoding: 8bit encoding
\usepackage[T1]{fontenc}
% input encoding: utf8 support
\usepackage[utf8]{inputenc}
% language settings: British English, New German
\usepackage{babel}

\usepackage{numprint}
%\usepackage{csquotes}

% Latin Modern font
\usepackage{lmodern}
% palatino "sans-"serif font
\renewcommand{\sfdefault}{ppl}
% extra math font
\usepackage{dsfont}
% another teletype font
\usepackage[nott]{inconsolata}
\def\consolata#1{\begingroup\fontfamily{zi4}\selectfont{#1}\endgroup}

% dagger symbols
\usepackage{textcomp}

\usepackage{textcomp}

% math symbols
\usepackage{amsmath,amsfonts,amssymb}
% small fractions in running text
\usepackage{nicefrac}
% text symbols
\usepackage{textcomp}
% extra math tools
\usepackage{mathtools}
% better arrays
\usepackage{array}
% better tabulars
\usepackage{tabularx,longtable}
% for tabulars with footnotes
\usepackage[flushleft]{threeparttable}
% for rotate tables
\usepackage{rotating}
% \begin{commment}
\usepackage{verbatim}
% latex hacks, e.g. robustify
\usepackage{etoolbox}
% arithmetic
\usepackage{calc}
% \hdashline
\usepackage{arydshln}
% varwidth paragraphs
\usepackage{varwidth}
% after page
\usepackage{afterpage}

% nicer text layout
\usepackage{microtype}

% allow graphics
\usepackage{graphicx}

% allow colors
\usepackage{xcolor}

\usepackage{tabstackengine}

% adaptive whitespace
\usepackage{xspace}

% chapter headers
\usepackage[explicit]{titlesec}

% allow hyperlinks
\usepackage{hyperref}
% setup hyperref
\hypersetup{
  pdftitle={High-Quality Hypergraph Partitioning},
  pdfauthor={Sebastian Schlag},
  pdfsubject={hypergraphs, hypergraph partitioning, dissertation},
  % hyperlinks in original color
  colorlinks=false,
  % hyperlinks without border
  pdfborder={0 0 0},
  % open all bookmark folders
  bookmarksopen=true,
  % enumerate bookmarks
  bookmarksnumbered=true,
  % allow links to line break
  breaklinks=true,
  unicode=true
}
\providecommand\phantomsection{} 

\makeatletter 
\newcommand{\textlabel}[2]{% 
  \protected@edef\@currentlabel{#1}% Set target label 
  \phantomsection% Correct hyper reference link 
  #1\label{#2}% Print and store label 
} 
\makeatother 

% change chapter counters to reset within each part
% \usepackage{chngcntr}
% \counterwithin{chapter}{part}

% page layout
\usepackage{scrpage2}
% \usepackage{scrlayer-scrpage}
% better integration of hyperref, listings, float
\usepackage{scrhack}

% loading package recommended by biblatex
\usepackage{csquotes}

% place floats exactly here [H]
\usepackage{float}
% fraction of page for top floats
\renewcommand{\topfraction}{0.8}
\renewcommand{\floatpagefraction}{0.8}

% caption for sub-elements
\usepackage[font=normalsize, labelformat=simple, list=true]{subcaption}
\renewcommand\thesubfigure{\,(\alph{subfigure})}

\usepackage{pdflscape}

% nicer tables
\usepackage{booktabs}
% table cells spanning rows
\usepackage{multirow}

% break long citations
\usepackage{breakcites}


% nice listings
% \usepackage[chapter]{algorithm}
% general settings for pseudo-code algorithms
% \usepackage{algpseudocode}

% fix for standalone drawing: add chapter counter
\ifstandalone
  \newcounter{chapter}
\fi

\ifstandalone\else

% algorithm formatting
% ours:
\usepackage[
% environment is algorithm2e instead of algorithms and \listofalgorithmes
algo2e,
% algo numbering within part, chapter or section
algochapter,
% layout of the algorithm
ruled,vlined,
% auto numbering of the algorithm's lines
linesnumbered,
% don't use relsize package (useful if it breaks the compatibily)
norelsize]{algorithm2e}
\DontPrintSemicolon
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}
\SetProgSty{}
\SetFuncSty{}
\SetArgSty{}
\def\listalgorithmcfname{List of Algorithms}
\def\algorithmautorefname{Algorithm}

% alias \tcp*{} to \Rem{} for pseudo-code comments, who knows what tcp* stands for?
\newcommand{\Rem}[1]{\tcp*{#1}}
% for pseudo-code comments inside () clauses, without line break
\newcommand{\Remi}[1]{\tcp*[f]{#1}}
% change C++ comments formatting
\SetKwComment{tcp}{{\upshape{}/\!/}\,}{}%
\SetCommentSty{textit}

% Custom pseudo-code functions
\SetKwProg{Function}{Function}{}{}
\SetKwFunction{LCPCompare}{LCP-Compare}

% C/C++ style increment and decrement (with nicer styling)
\newcommand{\Inc}{{++}}
\newcommand{\Dec}{{--}}

\fi

\usepackage{totcount}
\newtotcounter{citnum} %From the package documentation
\def\oldbibitem{} \let\oldbibitem=\bibitem
\def\bibitem{\stepcounter{citnum}\oldbibitem}

% listings
\usepackage{listings}
\lstset{
  language=C++,
  columns=fullflexible,
  basicstyle={\ttfamily},
  keywordstyle={\bfseries\color{dblue}},
  emphstyle={\color{dred}},
  aboveskip=0pt,
  belowskip=0pt,
}

\AtBeginDocument{%
  \renewcommand{\thelstlisting}{\arabic{chapter}.\arabic{lstlisting}}%
}

% Timo's TODOs
\newcommand{\TODO}[1]{%
  %{\sffamily\textbf{TODO}}%
  {{\sffamily\textbf{TODO}}[\textcolor{red}{\textit{#1}}]}%
  \marginpar{%
    %\raggedright\footnotesize\itshape{#1}\par%
    \raggedright\sffamily\textcolor{red}{\textbf{TODO}}\par%
  }}

% % format colon nicely in math typeset
% \mathchardef\ordinarycolon\mathcode`\:
% \mathcode`\:=\string"8000
% \begingroup \catcode`\:=\active
% \gdef:{\mathrel{\mathop\ordinarycolon}}
% \endgroup

% change \footnote{} style to use symbols
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}

% a command to print the footnote symbols, no idea why this does not exist.
\makeatletter
\newcommand{\fnsym}[1]{%
  \@fnsymbol{#1}%
}
\makeatother

% \textvtt{abc} - variable-width teletype with nicer literal underscores
\begingroup
\catcode`_=\active
\gdef\ActivateUnderscore{%
  % magic to replace underscore with a macro
  \def_{\texttt{\textunderscore}}%
  \catcode`\_=\active
}
\endgroup
\gdef\textvtt#1{%
  \begingroup\text{%
    \ActivateUnderscore{%
      \fontfamily{lmvtt}\selectfont{%
        \scantokens{#1\endinput}}}}%
  \endgroup}

%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%    Custom Layout Settings                                                    %

% do not uppercase all \markleft{} and \markboth{} page titles
\def\MakeMarkcase#1{#1}

% ---[ Part ]-------------------------------------------------------------------

%\definecolor{chaptergrey}{rgb}{0.6,0,0}
\definecolor{chaptergrey}{rgb}{0,0,0}

\newenvironment{savequote}[1][10cm]{%
  \begin{lrbox}{\quotebox}
    \begin{minipage}[t]{#1}\footnotesize\itshape\ignorespaces}{%
      \unskip\end{minipage}\end{lrbox}
  \global\setbox\quotebox\copy\quotebox
  \ignorespacesafterend}
\newcommand{\qauthor}[1]{%
  \par\smallskip
  {\raggedleft\upshape #1\qquad\hbox{}\par}\bigskip}
\newcommand{\qsetcnfont}[1]{%
    \renewcommand*{\defaultcnfont}{#1}}
\newsavebox{\quotebox}

\newenvironment{partabstract}[1][0.9\textwidth]{%
  \begin{lrbox}{\partabstractbox}
    \begin{minipage}[t]{#1}\normalfont\itshape\ignorespaces}{%
      \unskip\end{minipage}\end{lrbox}
  \global\setbox\partabstractbox\copy\partabstractbox
  \ignorespacesafterend}
\newsavebox{\partabstractbox}

\titleformat{name=\part}[display]{%
  % format:
  \thispagestyle{empty}\enlargethispage{2cm}}{%
  % label:
  \vbox to 110pt{\copy\quotebox\vss}%
  \vbox{%
    \raggedleft
    \fontfamily{ppl}\fontsize{100}{100}\selectfont
    \hfill\textcolor{chaptergrey}{\thepart}\newline
    \hfill\bfseries\fontfamily{ppl}\fontsize{20}{26}\selectfont#1%
  }
  \vspace{3em}
  \vbox{\centerline{\copy\partabstractbox}}%
}{%
  % sep:
  0pt}{%
  % before-body-code:
  \vspace{1pc}%
}
\titlespacing*{\part}{0pt}{0pt}{0pt}

\def\cleardoublepageblank{
  \clearpage%
  \ifodd\value{page}%
    % if already right, add blank page
    \hbox{}\clearpage\thispagestyle{empty}%
  \fi%
}

\let\oldpart\part
\renewcommand{\part}{\cleardoublepageblank\oldpart}

% ---[ Chapter ]----------------------------------------------------------------

% initial definitions of the chapter info (name and number)
\def\thischaptertitle{}\def\thischapternumber{}
\newtoggle{noFigs}

\newcommand\doSingleLine[1]{%
  \begingroup\let\newline=\ #1\endgroup%
}

\titleformat{name=\chapter}[display]{
  % format/label/sep:
  \sffamily\bfseries\fontsize{20}{22}\selectfont}{}{0pt}{
  % before-body-code:
  \begingroup
  \setlength{\unitlength}{1mm}
  \renewcommand{\gobble}[1]{}
  \begin{picture}(25,0)(0,5)
    \ifnumless{\thechapter}{10}{%
      \put(0,15){\line(1,0){\dimexpr\textwidth-15\unitlength\relax\gobble}}%
    }{%
      \put(0,15){\line(1,0){\dimexpr\textwidth-30\unitlength\relax\gobble}}
    }
    \put(100,1){\makebox(30,20)[r]{%
        \fontsize{72}{72}\selectfont\thechapter}}
    \put(0,15){%
      \makebox(\dimexpr\textwidth-20\unitlength\relax\gobble,\ht\strutbox\gobble)[l]{%
        \normalsize\chapapp~\thechapter}}
    \ifnumless{\thechapter}{10}{%
      \put(3,10){\parbox[t]{%
          \dimexpr\textwidth-19\unitlength\relax}{\raggedright\color{black} #1}}
    }{
      \put(3,10){\parbox[t]{%
          \dimexpr\textwidth-34\unitlength\relax}{\raggedright\color{black} #1}}
    }
  \end{picture}
  \endgroup
  % save chapterinfo
  \gdef\thischaptertitle{\doSingleLine{#1}}\gdef\thischapternumber{\thechapter}%
  \global\toggletrue{noFigs}
}
\titleformat{name=\chapter,numberless}[display]{
  % numberless are marked on both
  \markboth{#1}{#1}%
  % format/label/sep:
  \sffamily\bfseries\fontsize{20}{22}\selectfont}{}{0pt}{
  % before-body-code:
  \begingroup
  \vbox{%
    \raggedleft #1%
  }
  \endgroup
}

\titlespacing{name=\chapter}{0pt}{0pt}{40pt}
\titlespacing{name=\chapter,numberless}{0pt}{0pt}{20pt}

\makeatletter
% environment for chapter abstracts
\newenvironment{chapterabstract}{
  \bgroup
  \itshape
  \list{}{\leftmargin0.75cm\rightmargin\leftmargin}
\item\relax
}{
  \endlist
  \@afterindentfalse
  \@afterheading
  \egroup
}
\makeatother

% ---[ Paragraph ]--------------------------------------------------------------

\titleformat{\paragraph}[runin]{%
  \normalfont\normalsize\bfseries}{\theparagraph}{0em}{#1.}{}
\titlespacing*{\paragraph}{0pt}{\medskipamount}{1em}

% header / footer style
\ifstandalone\else
  \pagestyle{scrheadings}
  \setkomafont{pageheadfoot}{\normalfont\rmfamily}
  \setkomafont{pagenumber}{\normalfont\rmfamily}
  \setheadsepline{.4pt}
  \automark[section]{chapter}
\fi

% nicer captions
\usepackage{caption}

% caption style (general)
\captionsetup*{
  format=plain,
  labelfont={bf,up},
  margin=10pt,
}

% caption style (sub-elements)
\captionsetup*[sub]{
  format=plain,
  labelfont={bf,up},
  margin=10pt,
  skip=2pt
}

\usepackage{mdframed}
\definecolor{grisframe}{gray}{0.95}
\newmdenv[
  topline=false,
  bottomline=false,
  rightline=false,
  linewidth=3pt,
  linecolor=gray,
  innertopmargin=0pt,
  innerbottommargin=0pt,
  splitbottomskip=0pt,
  skipabove=.5\baselineskip,
  skipbelow=.5\baselineskip
]{siderules}

% ---[ better array column types ]----------------------------------------------

\newcolumntype{L}[1]{>{%
    \raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{%
    \centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{%
    \raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcolumntype{Y}{>{%
    \raggedleft\arraybackslash}X}

\newcolumntype{H}{@{}>{\iffalse}l<{\fi}}

% ---[ better enumerations ]----------------------------------------------------

\usepackage{enumitem}

% smaller margin for list environments
\setlist[itemize]{leftmargin=1.5em}
\setlist[enumerate]{leftmargin=1.5em}
\setlist[description]{leftmargin=1.5em}

\setlist[itemize]{topsep=0pt, labelsep=1ex}
\setlist[enumerate]{topsep=0pt, labelsep=1ex}
\setlist[description]{font=\normalfont,topsep=0pt}

\setlist[enumerate,1]{label=(\roman*), ref={\thetheorem\,(\roman*)}}
\setlist[enumerate,2]{label=(\alph*), ref={\thetheorem\,(\alph*)}}


% ---[ flow symbols ]----------------------------------------------------
\usepackage{stmaryrd}


% ---[ Add Chapter Splitting to Lists of Things ]-------------------------------

\makeatletter

\newcommand{\DeclareDividedList}[1]%
  {\newcounter{#1@chapter}\setcounter{#1@chapter}{0}}

\pretocmd{\addcontentsline}%
  {\ifltxcounter{#1@chapter}%
   {%
     \ifnumgreater{\thechapter}{\value{#1@chapter}}{%
       \setcounter{#1@chapter}{\thechapter}%
       \addtocontents{#1}{\protect\contentsline{chapter}%
         {\protect\numberline {\thechapter} {\thischaptertitle}}{}{} }
     }{}%
   }{}%
  }{}{}
\makeatother

\DeclareDividedList{lof}
\DeclareDividedList{lot}
\DeclareDividedList{loa}
\DeclareDividedList{thm}

\makeatother




%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%                                                                              %

% ---[ Macros ]-----------------------------------------------------------------

% round up
\newcommand{\ceil}[1]{\ensuremath{\lceil #1 \rceil}}
% roundd down
\newcommand{\floor}[1]{\ensuremath{\lfloor #1 \rfloor}}

% \arr{...} denotes an (ordered) array
\newcommand{\arr}[1]{[\, #1 \,]}
% \arrc{...} denotes an (ordered) array with less space
\newcommand{\arrc}[1]{[#1]}
% \arro{...} denotes an (ordered) right-open array
\newcommand{\arro}[1]{[\, #1 \kern.1em )}
% \set{...} denotes an (unordered) set
\newcommand{\set}[1]{\left\{ #1\right\}}
% \seq{...} sequence <...>
\newcommand{\seq}[1]{\left\langle #1\right\rangle}

% Landau Big-O
\newcommand{\Oh}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\oh}[1]{\ensuremath{\mathrm{o}(#1)}\xspace}
\newcommand{\Om}[1]{\ensuremath{\Omega(#1)}\xspace}
\newcommand{\om}[1]{\ensuremath{\omega(#1)}\xspace}
\newcommand{\Th}[1]{\ensuremath{\Theta(#1)}\xspace}

% Landau Big-O vertically expanding
\newcommand{\vOh}[1]{\ensuremath{\mathcal{O}\left(#1\right)}\xspace}
\newcommand{\voh}[1]{\ensuremath{\mathrm{o}\left(#1\right)}\xspace}
\newcommand{\vOm}[1]{\ensuremath{\Omega\left(#1\right)}\xspace}
\newcommand{\vom}[1]{\ensuremath{\omega\left(#1\right)}\xspace}
\newcommand{\vTh}[1]{\ensuremath{\Theta\left(#1\right)}\xspace}

% mathmatical operators
\newcommand{\xor}{\mathbin{\oplus}}

\def\mathsc#1{\ensuremath{\text{\textsc{#1}}}}


%\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{wasysym}
\newcommand{\no}{$\Circle$}%
\newcommand{\yes}{$\CIRCLE$}%
\newcommand{\yesno}{$\LEFTcircle$}
\newcommand{\ymark}{\ding{51}}%


\newcommand{\Partition}{\ensuremath{\mathrm{\Pi}}}%
\newcommand{\neighbors}{\ensuremath{\mathrm{\Gamma}}}%
\newcommand{\incnets}{\ensuremath{\mathrm{I}}}%
\newcommand{\pinsinpart}{\ensuremath{\mathrm{\Phi}}}
\newcommand{\adjblocks}{\ensuremath{\mathrm{B}}}
\newcommand{\con}{\ensuremath{\lambda}}
\newcommand{\conset}{\ensuremath{\Lambda}}
\newcommand{\frompart}{\ensuremath{V_{\text{\upshape from}}}}
\newcommand{\topart}{\ensuremath{V_{\text{\upshape to}}}}
\newcommand{\frompq}{\ensuremath{P_{\text{\upshape from}}}}
\newcommand{\topq}{\ensuremath{P_{\text{\upshape to}}}}
\newcommand{\fromgain}{\ensuremath{g_{\text{\upshape from}}}}
\newcommand{\togain}{\ensuremath{g_{\text{\upshape to}}}}

\newcommand{\maxdeg}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\maxsize}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\avgdeg}{\ensuremath{\overline{d(v)}}}
\newcommand{\avgsize}{\ensuremath{\overline{|e|}}}
\newcommand{\meddeg}{\ensuremath{\widetilde{d(v)}}}
\newcommand{\medsize}{\ensuremath{\widetilde{|e|}}}

\newcommand{\objective}{\ensuremath{\mathfrak{O}}}%
\newcommand{\ocut}{\ensuremath{\mathfrak{f}_c(\Partition)}}%
\newcommand{\ocon}{\ensuremath{\mathfrak{f}_\lambda(\Partition)}}%
\newcommand{\osoed}{\ensuremath{\mathfrak{f}_s(\Partition)}}%
\newcommand{\orc}{\ensuremath{\mathfrak{f}_{rc}(\Partition)}}%
\newcommand{\osc}{\ensuremath{\mathfrak{f}_{sc}(\Partition)}}%


\SetKw{Continue}{continue}
\SetKwFunction{Activate}{Activate}
\SetKwFunction{rate}{rate}
\SetKwFunction{coarsen}{coarsen}
\SetKwFunction{DeltaGainUpdate}{DeltaGainUpdate}
\SetKwFunction{UpdateGainCache}{UpdateGainCache}

\usepackage{etoolbox,siunitx}
\sisetup{detect-weight=true,detect-inline-weight=math}
\robustify\bfseries

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\ALL}{All}
\newcommand{\Dual}{Dual}
\newcommand{\Primal}{Primal}
\newcommand{\ISPD}{ISPD98}
\newcommand{\Literal}{Literal}
\newcommand{\SPM}{SPM}
\newcommand{\DAC}{DAC2012}

\newcommand{\KaHyPar}[1]{KaHyPar-#1}
\newcommand{\KaHyParConfig}[2]{KaHyPar-#1$_\text{(#2)}$}
\newcommand{\hMetis}[1]{hMetis-#1}
\newcommand{\PaToH}[1]{PaToH-#1}

\newcommand{\FlowVariant}[3]{($#1$\text{F},$#2$\text{M},$#3$\text{LS})}
\newcommand{\Constant}[1]{\textsc{Constant#1}}


\DeclareMathOperator*{\argmax}{arg\,max}%

\newcommand*\rot{\rotatebox{90}}
%\newcommand*\OK{\ding{51}}
\newcommand*\OK{\yes}
% \newcommand{\NOK}{\ding{55}}%
\newcommand{\NOK}{\no}%

% \usepackage{relsize}
% https://tex.stackexchange.com/questions/4302/prettiest-way-to-typeset-c-cplusplus
% \newcommand\CC{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}}
\newcommand\CC{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}}

\usepackage{relsize}
\renewcommand{\_}{\textscale{.7}{\textunderscore}}

%https://tex.stackexchange.com/questions/41787/use-textwidth-for-image-width-only-when-it-outgrows-the-page
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox


% ---[ Theorem Environments ]---------------------------------------------------

\usepackage[amsmath,thmmarks,hyperref]{ntheorem}

% \renewtheoremstyle{break}%
%   {\labelsep=0pt\item[\rlap{\vbox{\hbox to \textwidth{\upshape\bfseries ##1\ ##2\hskip 0pt plus 1fil}\hbox{\strut}}}]}%
%   {\labelsep=0pt\item[\rlap{\vbox{\hbox to \textwidth{\upshape\bfseries ##1\ ##2\ (##3\unskip)\hskip 0pt plus 1fil}\hbox{\strut}}}]}

\renewtheoremstyle{nonumberplain}%
  {\labelsep=0pt\item[\itshape ##1.\quad]}%
  {\labelsep=0pt\item[\itshape ##1.\ (##3)\quad]}

\theoremstyle{break}
\theorembodyfont{\itshape}
\theoremseparator{\smallskip}
\theorempreskip{\bigskipamount}
\theorempostskip{\medskipamount}

\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{observation}[theorem]{Observation}

% proof environment
\theoremstyle{nonumberplain}
\theoremheaderfont{\itshape}
\theoremsymbol{\ensuremath{\;\square}}
\theorempreskip{}
\theorempostskip{}
\theorembodyfont{\normalfont}
\newtheorem{proof}{Proof}

% make text in \textbf{} also bold in math mode
\makeatletter
\DeclareRobustCommand*{\bfseries}{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont
  \boldmath\let\mathbbnormal=\mathbb\let\mathbb=\mathbbm
}
\makeatother

% ---[ CleverRef ]--------------------------------------------------------------

% use cleveref
\usepackage[noabbrev]{cleveref}
\crefname{algocf}{algorithm}{algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}

\crefname{conjecture}{conjecture}{conjectures}
\crefname{observation}{observation}{observations}

% disable hyperref
\let\autoref\undefined

% cleveref options for enumi: remove "item "
\crefformat{enumi}{#2#1#3}

% i like "1--2" better than "1 to 2"
\newcommand{\crefrangeconjunction}{--}

%                                                                              %
%%                                                                            %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                            %%
%    Bibliography                                                              %

% use biblatex
\usepackage[
  backend=biber,
  style=alphabetic,
  sorting=ynt,
  language=english,
  backref,
  sortcites,
  abbreviate=false,
  maxnames=4,
  minnames=1,
  maxbibnames=9999,
  maxcitenames=2,
  citetracker=true,
  defernumbers=true,
  labelnumber
  ]{biblatex}

%https://tex.stackexchange.com/questions/48846/biblatex-et-al-beginning-from-second-citation
\AtEveryCitekey{\ifciteseen{}{\defcounter{maxnames}{99}}}

%https://tex.stackexchange.com/questions/311426/bibliography-error-use-of-blxbblverbaddi-doesnt-match-its-definition-ve
\makeatletter
\def\blx@maxline{77}
\makeatother
  
% bib file
\addbibresource{references.bib}
\addbibresource{publications.bib}

\DefineBibliographyStrings{english}{%
  backrefpage = {see~page},
  backrefpages = {see~pages},
  mathesis = {Master Thesis},
}

%https://tex.stackexchange.com/questions/299064/biblatex-two-bibliographies-with-different-styles-and-sortings
%Append keywords to identify different bibliography entries.
\DeclareSourcemap{
  \maps[datatype=bibtex, overwrite]{
    \map{
      \perdatasource{references.bib}
      \step[fieldset=KEYWORDS, fieldvalue=primary, append]
    }
    \map{
      \perdatasource{publications.bib}
      \step[fieldset=KEYWORDS, fieldvalue=secondary, append]
    }
  }
}

\DeclareFieldFormat{labelnumberwidth}{\mkbibbrackets{#1}}
\renewbibmacro*{cite}{%
  \printtext[bibhyperref]{%
    \printfield{labelprefix}%
    \ifkeyword{secondary}
      {\printfield{labelnumber}}
      {\printfield{labelalpha}%
       \printfield{extraalpha}}}}


\defbibenvironment{bibliographyNUM}
  {\list
     {\printtext[labelnumberwidth]{%
        \printfield{prefixnumber}%
        \printfield{labelnumber}}}
     {\setlength{\labelwidth}{\labelnumberwidth}%
      \setlength{\leftmargin}{\labelwidth}%
      \setlength{\labelsep}{\biblabelsep}%
      \addtolength{\leftmargin}{\labelsep}%
      \setlength{\itemsep}{\bibitemsep}%
      \setlength{\parsep}{\bibparsep}}%
      \renewcommand*{\makelabel}[1]{\hss##1}}
  {\endlist}
  {\item}

\assignrefcontextkeyws[sorting=none]{secondary}

\usepackage{pbox}

\DeclareFieldFormat{pagerefformat}{%
  \begingroup%
  \hspace{1ex plus 1fill}\penalty500%
  \hspace*{\fill}%
  \pbox[t]{.7\textwidth}{\raggedleft\small\textcolor{gray}{[#1]}}%
  \endgroup%
}

\renewbibmacro*{pageref}{%
  % dot after every bibliography entry
  .%
  \iflistundef{pageref}{%
  }{%
    \printtext[pagerefformat]{%
      \ifnumgreater{\value{pageref}}{1}{%
        \bibstring{backrefpages}\ppspace%
      }{%
        \bibstring{backrefpage}\ppspace%
      }%
      \printlist[pageref][-\value{listtotal}]{pageref}%
    }%
  }%
}

% the punctuation printed at the very end of every bibliography entry
\renewcommand{\finentrypunct}{}

% ------------------------------------------------------------------------------
% TikZ
\usepackage{tikz}

\usetikzlibrary{arrows.meta}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{chains}
\usetikzlibrary{decorations}
\usetikzlibrary{fit}
\usetikzlibrary{matrix}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.callouts}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.symbols}


% glossary, symbols, acronyms
\usepackage[toc, nomain]{glossaries}


\newcommand*{\skippingparagraph}{\par\vspace{.5\baselineskip}\noindent}


\newcommand{\add}[1]{\textcolor{blue}{#1}}
